Preference-Conditioned Gradient Variations for Multi-Objective Quality-Diversity

In a variety of domains, from robotics to finance, Quality-Diversity algorithms have been used to generate collections of both diverse and high-performing solutions. Multi-Objective Quality-Diversity algorithms have emerged as a promising approach for applying these methods to complex, multi-objective problems. However, existing methods are limited by their search capabilities. For example, Multi-Objective Map-Elites depends on random genetic variations which struggle in high-dimensional search spaces. Despite efforts to enhance search efficiency with gradient-based mutation operators, existing approaches consider updating solutions to improve on each objective separately rather than achieving desired trade-offs. In this work, we address this limitation by introducing Multi-Objective Map-Elites with Preference-Conditioned Policy-Gradient and Crowding Mechanisms: a new Multi-Objective Quality-Diversity algorithm that uses preference-conditioned policy-gradient mutations to efficiently discover promising regions of the objective space and crowding mechanisms to promote a uniform distribution of solutions on the non-dominated front. We evaluate our approach on six robotics locomotion tasks and show that our method outperforms or matches all state-of-the-art Multi-Objective Quality-Diversity methods in all six, including two newly proposed tri-objective tasks. Importantly, our method also achieves a smoother set of trade-offs, as measured by newly-proposed sparsity-based metrics.

==> Results/figures/ablations_sparsity.tex <==
\begin{table*}[ht]
\centering
  \caption{Ablations Sparsity Metrics Results}
  \scalebox{0.9}{\begin{tabular}{ p{2cm}| p{1.05cm} | p{1.45cm} | p{1.45cm} | p{1.45cm} | p{1.45cm} | p{1.45cm} | p{1.45cm} | p{1.45cm}}
  
    \toprule

    \multicolumn{2}{c|}{ }&
    \pcc &
    \injectactor &
    \nopg &
    \nocrowding &
    \keeppref &
    \onehot &
    \randomactor
    \\

    \midrule
    \midrule
    
    \multirow{2}{*}{\textsc{Ant-2}}& 
    QD-S&
    &
    &
    &
    &
    &
    &
    \\

    & 
    Global-S&
    &
    &
    &
    &
    &
    &
    \\

    \midrule
    
    \multirow{2}{*}{\textsc{Ant-3}}& 
    QD-S&
    &
    &
    &
    &
    &
    &
    \\

    & 
    Global-S&
    &
    &
    &
    &
    &
    &
    \\

    \midrule
    
    \multirow{2}{*}{\textsc{HalfCheetah-2}}& 
    QD-S&
    &
    &
    &
    &
    &
    &
    \\

    & 
    Global-S&
    &
    &
    &
    &
    &
    &
    \\

    \midrule
    
    \multirow{2}{*}{\textsc{Hopper-2}}& 
    QD-S&
    &
    &
    &
    &
    &
    &
    \\

    & 
    Global-S&
    &
    &
    &
    &
    &
    &
    \\

    \midrule
    
    \multirow{2}{*}{\textsc{Hopper-3}}& 
    QD-S&
    &
    &
    &
    &
    &
    &
    \\

    & 
    Global-S&
    &
    &
    &
    &
    &
    &
    \\  

    \midrule

    \multirow{2}{*}{\textsc{Walker2d-2}}& 
    QD-S&
    &
    &
    &
    &
    &
    &
    \\

    & 
    Global-S&
    &
    &
    &
    &
    &
    &
    \\
    
    \bottomrule
    
  \end{tabular}}
  \label{tab:sparsity_ablations_results}
\end{table*}

